Universal Approximation with Certified Networks

Training neural networks to be certifiably robust is critical to ensure their safety against adversarial attacks. However, it is currently very difficult to train a neural network that is both accurate and certifiably robust. In this work we take a step towards addressing this challenge. We prove that for every continuous function $f$, there exists a network $n$ such that: (i) $n$ approximates $f$ arbitrarily close, and (ii) simple interval bound propagation of a region $B$ through $n$ yields a result that is arbitrarily close to the optimal output of $f$ on $B$. Our result can be seen as a Universal Approximation Theorem for interval-certified ReLU networks. To the best of our knowledge, this is the first work to prove the existence of accurate, interval-certified networks.

==> figures/neighborhood.tex <==
\begin{tikzpicture}[scale=0.5, every node/.style={scale=0.8}]
    \pgfmathsetmacro{\l}{1.5}
    \pgfmathsetmacro{\h}{3}
    
    \foreach \i in {1,...,4}
        \foreach \j in {1,...,4} {
            \coordinate (\j \i) at (\i * \l, \j * \l);
        }

    \coordinate (c) at (3 * \l, \h, 3 * \l);
    

    \foreach \i in {1,...,3}
        \foreach \j in {1,...,4} {
            \draw[dotted] (\i * \l, \j * \l) -- (\i * \l + \l, \j * \l);
        }
    
    \foreach \i in {1,...,4}
        \foreach \j in {1,...,3} {
            \draw[dotted] (\i * \l, \j * \l) -- (\i * \l, \j * \l + \l);
        }
    
    \draw[blue] (3.45 * \l, 3.45 * \l) -- (3.55 * \l, 3.55 * \l);
    \draw[blue] (3.45 * \l, 3.55 * \l) -- (3.55 * \l, 3.45 * \l);
    \node[blue] at (3.7 * \l, 3.5 * \l){$x$};

    \node at (3 * \l, 3 * \l)[circle,fill=blue,inner sep=1.5pt]{};
    \node at (3 * \l, 4 * \l)[circle,fill=blue,inner sep=1.5pt]{};
    \node at (4 * \l, 3 * \l)[circle,fill=blue,inner sep=1.5pt]{};
    \node at (4 * \l, 4 * \l)[circle,fill=blue,inner sep=1.5pt]{};

    \node[red] at (2.5 * \l, 1.5 * \l){$U$};

    \node at (1 * \l, 1 * \l)[circle,fill=red,inner sep=1.5pt]{};
    \node at (2 * \l, 1 * \l)[circle,fill=red,inner sep=1.5pt]{};
    \node at (3 * \l, 1 * \l)[circle,fill=red,inner sep=1.5pt]{};
    \node at (1 * \l, 2 * \l)[circle,fill=red,inner sep=1.5pt]{};
    \node at (2 * \l, 2 * \l)[circle,fill=red,inner sep=1.5pt]{};
    \node at (3 * \l, 2 * \l)[circle,fill=red,inner sep=1.5pt]{};

    
    \draw [red] plot [smooth cycle] coordinates {
        (1.3*\l, 1.2*\l) 
        (1.1*\l, 1.5*\l)
        (1.3*\l, 1.8*\l) 
        (2*\l, 1.7*\l)
        (2.7*\l, 1.8*\l)
        (2.9*\l, 1.5*\l)
        (2.7*\l, 1.2*\l)
        (2*\l, 1.3*\l)};

\end{tikzpicture}  

